Exact and Semiclassical Density Matrix of a Particle Moving in a Barrier Potential with Bound States

We present a barrier potential with bound states that is exactly solvable and determine the eigenfunctions and eigenvalues of the Hamiltonian. The equilibrium density matrix of a particle moving at temperature T in this nonlinear barrier potential field is determined. The exact density matrix is compared with the result of the path integral approach in the semiclassical approximation. For opaque barriers the simple semiclassical approximation is found to be sufficient at high temperatures while at low temperatures the fluctuation paths may have a caustic depending on temperature and endpoints. Near the caustics the divergence of the simple semiclassical approximation of the density matrix is removed by a nonlinear fluctuation potential. For opaque barriers the improved semiclassical approximation is again in agreement with the exact result. In particular, bound states and the form of resonance states are described accurately by the semiclassical approach.

==> fig11.tex <==
%auto-ignore

\begin{figure}[t]
%\flushright
\begin{center}
\vskip-0.8cm
\leavevmode
\epsfxsize=15cm
\epsffile{geb.eps}
\end{center}
\end{figure}



==> fig5.tex <==
%auto-ignore

\begin{figure}
%\flushright
\begin{center}
\vskip-0.8cm
\leavevmode
\epsfxsize=15cm
\epsffile{abif.eps}
\end{center}
%\vskip-0.5cm
\label{fig:bif}
\end{figure}


==> fig6.tex <==
%auto-ignore

\begin{figure}
%\flushright
\begin{center}
\vskip-0.8cm
\leavevmode
\epsfxsize=14cm
\epsffile{p1.eps}
\end{center}
%vskip-1cm
\label{fig:hightc}
\end{figure}
	
